Arabic Fine-Grained Entity Recognition

Traditional NER systems are typically trained to recognize coarse-grained entities, and less attention is given to classifying entities into a hierarchy of fine-grained lower-level subtypes. This article aims to advance Arabic NER with fine-grained entities. We chose to extend Wojood (an open-source Nested Arabic Named Entity Corpus) with subtypes. In particular, four main entity types in Wojood, geopolitical entity (GPE), location (LOC), organization (ORG), and facility (FAC), are extended with 31 subtypes. To do this, we first revised Wojood's annotations of GPE, LOC, ORG, and FAC to be compatible with the LDC's ACE guidelines, which yielded 5, 614 changes. Second, all mentions of GPE, LOC, ORG, and FAC (~44K) in Wojood are manually annotated with the LDC's ACE sub-types. We refer to this extended version of Wojood as WojoodF ine. To evaluate our annotations, we measured the inter-annotator agreement (IAA) using both Cohen's Kappa and F1 score, resulting in 0.9861 and 0.9889, respectively. To compute the baselines of WojoodF ine, we fine-tune three pre-trained Arabic BERT encoders in three settings: flat NER, nested NER and nested NER with subtypes and achieved F1 score of 0.920, 0.866, and 0.885, respectively. Our corpus and models are open-source and available at https://sina.birzeit.edu/wojood/.

==> tables/nested_ner_results.tex <==
\begin{table}[H]
\centering
 \renewcommand{\arraystretch}{3}
\resizebox{1\columnwidth}{!}{%
% \resizebox{0.95\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{Test} & \multicolumn{2}{c|}{Finance} & \multicolumn{2}{c|}{Science} & \multicolumn{2}{c|}{Politics} \\
        \hline
        ARBERTv2 & MARBERTv2 & ARBERTv2 &MARBERTv2 & ARBERTv2 & MARBERTv2 & ARBERTv2 & MARBERTv2 \\
        \hline
        0.845 & 0.861 & 0.458 & 0.499 & 0.494 & 0.554 & 0.557 & 0.612 \\
        \hline
\end{tabular}
}
\caption{Nested NER results on test and new domains: politics, finance, and science.   }  
\label{tab:nested_ner_results}
\end{table}

==> tables/subtypes_ner_guidelines.tex <==
\begin{table}[h]
\begin{tabular}{p{1.5cm}|p{0.7cm}p{3.1cm}|p{0.7cm}}
\hline 
 \small Guideline & \small Classes  & \small Sub-type Classes  &  \small Arabic  \\ \hline 
 
 \small \href{https://doi.org/10.5281/zenodo.3604227}{Impresso}  &  \small 7
 &   \small 6 for Location and 2 for Organisation &  \small No  
\\ 

\small \href{https://grobid-ner.readthedocs.io/en/latest/class-and-senses/}{Grobid-ner}  &  \small 27
 &   \small - &  \small No  
\\ 
\small \href{https://www.cnts.ua.ac.be/conll2003/ner/annotation.txt}{CONLL-2003}  &  \small 4
 &   \small 9 under Location and 9 under Organisation &  \small No  
\\

\small \href{https://zenodo.org/record/4574199}{NewsEye}  &  \small 5
 &   \small 5 under Location and 2 under Organisation &  \small No  
\\
  
\small \href{https://www.ldc.upenn.edu/sites/www.ldc.upenn.edu/files/arabic-entities-guidelines-v7.4.2.pdf}{LDC's ACE guideline}  & \small 5 &  \small 11 under GPE, 7 under LOC, 9 under ORG, and 5 under FAC & \small YES
\\ \hline 

 \small Our Guideline  &
  \small 21 & \small 7 under GPE, 9 under LOC, 10 under ORG, and 5 under FAC & \small YES \normalsize
\\ \hline
\end{tabular}
\caption{Existing sub-typed NER  guidelines.\label{tab:tab1} }
\end{table} 
